Efficient Few-Shot Continual Learning in Vision-Language Models

Vision-language models (VLMs) excel in tasks such as visual question answering and image captioning. However, VLMs are often limited by their use of pretrained image encoders, like CLIP, leading to image understanding errors that hinder overall performance. On top of that, real-world applications often require the model to be continuously adapted as new and often limited data continuously arrive. To address this, we propose LoRSU (Low-Rank Adaptation with Structured Updates), a robust and computationally efficient method for selectively updating image encoders within VLMs. LoRSU introduces structured and localized parameter updates, effectively correcting performance on previously error-prone data while preserving the model's general robustness. Our approach leverages theoretical insights to identify and update only the most critical parameters, achieving significant resource efficiency. Specifically, we demonstrate that LoRSU reduces computational overhead by over 25x compared to full VLM updates, without sacrificing performance. Experimental results on VQA tasks in the few-shot continual learning setting, validate LoRSU's scalability, efficiency, and effectiveness, making it a compelling solution for image encoder adaptation in resource-constrained environments.

==> tables/lorsu_attn_vs_rand_all.tex <==

\begin{table}
\caption{Comparison of the importance of choosing a small subset of attention heads. \emph{LoRSU-RAND-V-CLIP} randomly chooses 2 heads to fine-tune, \emph{LoRSU-F} fine-tunes all the available heads, and our baseline \emph{LoRSU} that chooses the top-2 attentions heads. We report the accuracy scores (\%) for LLaVA with the pretrained or fine-tuned CLIP CLIP-L-14. All baselines use \textbf{GTS} dataset for fine-tuning the vision encoder(the LLM remains frozen). We include error bars over 3 runs.}
 \label{table:lorsu_attn_gtsrb_clip}
\begin{center}
\begin{small}
\begingroup
\setlength{\tabcolsep}{2.0pt}
\begin{tabular}{l c c c c c c c c c c c}
\toprule
 & & \multicolumn{9}{c}{\textbf{VQA Datasets (Acc \%)}}  \\
\cmidrule(lr){3-12}
\textbf{Setting} & \textbf{FT Method}  & \textbf{GTS} & \textbf{TSI} & \textbf{CAn} & \textbf{AIR} & \textbf{ESAT} & \textbf{DALLE} & \textbf{VSR} & \textbf{HM} & \textbf{MMVP} & \textbf{VisOnly} \\
\midrule
 & \textbf{Zr-Shot} & $75.6$ & $53.1$ & $82.7$ & $60.4$ & $76.1$ & $91.1$ & $51.5$ & $61.2$ & $58.0$ & $31.3$ \\
\midrule
\multirow{3}{*}{\textbf{CL-5}} & \textbf{LoRSU-Rand} & $81.2 \mtiny{\pm 1.2}$ & $53.5 \mtiny{\pm 0.5}$ & $82.2 \mtiny{\pm 0.6}$ & $61.2 \mtiny{\pm 1.2}$ & $65.0 \mtiny{\pm 0.9}$ & $90.4 \mtiny{\pm 1.3}$ & $51.8 \mtiny{\pm 1.5}$ & $61.7 \mtiny{\pm 1.1}$ & $58.2 \mtiny{\pm 0.2}$ & $32.1 \mtiny{\pm 0.4}$ \\
& \textbf{LoRSU-F} & $82.3 \mtiny{\pm 0.6}$ & $53.3 \mtiny{\pm 0.8}$ & $82.2 \mtiny{\pm 1.3}$ & $60.9 \mtiny{\pm 1.0}$ & $65.7 \mtiny{\pm 0.9}$ & $91.1 \mtiny{\pm 1.2}$ & $51.6 \mtiny{\pm 0.9}$ & $61.9 \mtiny{\pm 0.8}$ & $58.4 \mtiny{\pm 0.4}$ & $31.2 \mtiny{\pm 0.2}$ \\
& \textbf{LoRSU} & $81.8 \mtiny{\pm 0.6}$ & $53.4 \mtiny{\pm 1.3}$ & $82.6 \mtiny{\pm 0.7}$ & $61.0 \mtiny{\pm 1.4}$ & $66.6 \mtiny{\pm 1.4}$ & $91.4 \mtiny{\pm 1.1}$ & $51.7 \mtiny{\pm 1.4}$ & $61.6 \mtiny{\pm 0.6}$ & $59.8 \mtiny{\pm 0.4}$ & $31.4 \mtiny{\pm 0.4}$ \\
\midrule
\multirow{3}{*}{\textbf{CL-20}} & \textbf{LoRSU-Rand} & $83.1 \mtiny{\pm 0.5}$ & $53.4 \mtiny{\pm 0.9}$ & $82.6 \mtiny{\pm 0.3}$ & $60.8 \mtiny{\pm 0.8}$ & $61.2 \mtiny{\pm 0.5}$ & $90.5 \mtiny{\pm 0.9}$ & $51.7 \mtiny{\pm 0.8}$ & $61.7 \mtiny{\pm 0.8}$ & $59.4 \mtiny{\pm 0.2}$ & $32.2 \mtiny{\pm 0.2}$ \\
& \textbf{LoRSU-F} & $84.4 \mtiny{\pm 0.6}$ & $53.6 \mtiny{\pm 0.4}$ & $82.3 \mtiny{\pm 0.6}$ & $60.3 \mtiny{\pm 0.5}$ & $60.1 \mtiny{\pm 0.5}$ & $91.4 \mtiny{\pm 0.7}$ & $52.0 \mtiny{\pm 0.5}$ & $61.3 \mtiny{\pm 0.8}$ & $59.1 \mtiny{\pm 0.2}$ & $32.0 \mtiny{\pm 0.1}$ \\
& \textbf{LoRSU} & $84.3 \mtiny{\pm 0.9}$ & $53.2 \mtiny{\pm 1.0}$ & $82.4 \mtiny{\pm 0.4}$ & $60.7 \mtiny{\pm 0.6}$ & $64.5 \mtiny{\pm 0.4}$ & $90.8 \mtiny{\pm 0.8}$ & $52.0 \mtiny{\pm 0.4}$ & $62.1 \mtiny{\pm 0.9}$ & $59.5 \mtiny{\pm 0.2}$ & $31.7 \mtiny{\pm 0.1}$ \\
\midrule
\multirow{3}{*}{\textbf{CL-50}} & \textbf{LoRSU-Rand} & $84.5 \mtiny{\pm 0.3}$ & $54.2 \mtiny{\pm 0.3}$ & $81.8 \mtiny{\pm 0.1}$ & $60.8 \mtiny{\pm 0.4}$ & $57.2 \mtiny{\pm 0.2}$ & $90.9 \mtiny{\pm 0.4}$ & $51.7 \mtiny{\pm 0.1}$ & $61.3 \mtiny{\pm 0.4}$ & $60.4 \mtiny{\pm 0.0}$ & $31.9 \mtiny{\pm 0.0}$ \\
& \textbf{LoRSU-All} & $85.6 \mtiny{\pm 0.2}$ & $53.8 \mtiny{\pm 0.2}$ & $81.2 \mtiny{\pm 0.4}$ & $60.5 \mtiny{\pm 0.1}$ & $59.0 \mtiny{\pm 0.2}$ & $90.4 \mtiny{\pm 0.4}$ & $51.7 \mtiny{\pm 0.2}$ & $61.6 \mtiny{\pm 0.0}$ & $58.2 \mtiny{\pm 0.0}$ & $31.7 \mtiny{\pm 0.1}$ \\
& \textbf{LoRSU} & $85.2 \mtiny{\pm 0.3}$ & $53.8 \mtiny{\pm 0.2}$ & $81.8 \mtiny{\pm 0.3}$ & $60.8 \mtiny{\pm 0.4}$ & $61.6 \mtiny{\pm 0.2}$ & $90.9 \mtiny{\pm 0.1}$ & $51.9 \mtiny{\pm 0.3}$ & $62.1 \mtiny{\pm 0.4}$ & $59.0 \mtiny{\pm 0.1}$ & $31.7 \mtiny{\pm 0.1}$ \\
\bottomrule
\end{tabular}
\endgroup
\end{small}
\end{center}
\end{table}




\begin{table}
\caption{Comparison of the importance of choosing a small subset of attention heads. \emph{LoRSU-RAND-V-CLIP} randomly chooses 2 heads to fine-tune, \emph{LoRSU-F} fine-tunes all the available heads, and our baseline \emph{LoRSU} that chooses the top-2 attentions heads. We report the accuracy scores (\%) for LLaVA with the pretrained or fine-tuned CLIP CLIP-L-14. All baselines use \textbf{TSI} dataset for fine-tuning the vision encoder(the LLM remains frozen). We include error bars over 3 runs.}
 \label{table:lorsu_attn_tsi_clip}
\begin{center}
\begin{small}
\begingroup
\setlength{\tabcolsep}{2.0pt}
\begin{tabular}{l c c c c c c c c c c c}
\toprule
 & & \multicolumn{9}{c}{\textbf{VQA Datasets (Acc \%)}}  \\
\cmidrule(lr){3-12}
\textbf{Setting} & \textbf{FT Method}  & \textbf{GTS} & \textbf{TSI} & \textbf{CAn} & \textbf{AIR} & \textbf{ESAT} & \textbf{DALLE} & \textbf{VSR} & \textbf{HM} & \textbf{MMVP} & \textbf{VisOnly} \\
\midrule
 & \textbf{Zr-Shot} & $75.6$ & $53.1$ & $82.7$ & $60.4$ & $76.1$ & $91.1$ & $51.5$ & $61.2$ & $58.0$ & $31.3$ \\
\midrule
\multirow{3}{*}{\textbf{CL-5}} & \textbf{LoRSU-Rand} & $74.8 \mtiny{\pm 1.4}$ & $55.0 \mtiny{\pm 1.3}$ & $82.9 \mtiny{\pm 0.6}$ & $60.2 \mtiny{\pm 0.6}$ & $75.7 \mtiny{\pm 1.3}$ & $91.5 \mtiny{\pm 1.2}$ & $51.6 \mtiny{\pm 1.1}$ & $62.0 \mtiny{\pm 1.2}$ & $58.2 \mtiny{\pm 0.3}$ & $31.5 \mtiny{\pm 0.4}$ \\
& \textbf{LoRSU-F} & $75.8 \mtiny{\pm 1.3}$ & $55.7 \mtiny{\pm 0.5}$ & $83.1 \mtiny{\pm 1.4}$ & $60.5 \mtiny{\pm 0.6}$ & $75.8 \mtiny{\pm 1.0}$ & $91.6 \mtiny{\pm 1.3}$ & $51.9 \mtiny{\pm 0.8}$ & $61.7 \mtiny{\pm 1.5}$ & $57.7 \mtiny{\pm 0.4}$ & $31.9 \mtiny{\pm 0.3}$ \\
& \textbf{LoRSU} & $75.6 \mtiny{\pm 1.3}$ & $56.6 \mtiny{\pm 0.8}$ & $82.4 \mtiny{\pm 1.4}$ & $60.5 \mtiny{\pm 0.7}$ & $76.1 \mtiny{\pm 0.7}$ & $91.4 \mtiny{\pm 1.4}$ & $51.5 \mtiny{\pm 0.8}$ & $61.8 \mtiny{\pm 0.9}$ & $57.7 \mtiny{\pm 0.3}$ & $31.2 \mtiny{\pm 0.4}$ \\
\midrule
\multirow{3}{*}{\textbf{CL-20}} & \textbf{LoRSU-Rand} & $75.4 \mtiny{\pm 0.6}$ & $62.0 \mtiny{\pm 0.6}$ & $81.9 \mtiny{\pm 0.7}$ & $59.1 \mtiny{\pm 0.8}$ & $73.5 \mtiny{\pm 0.4}$ & $90.6 \mtiny{\pm 0.4}$ & $51.9 \mtiny{\pm 0.5}$ & $62.1 \mtiny{\pm 0.7}$ & $58.1 \mtiny{\pm 0.2}$ & $31.4 \mtiny{\pm 0.2}$ \\
& \textbf{LoRSU-F} & $75.2 \mtiny{\pm 0.9}$ & $63.1 \mtiny{\pm 0.6}$ & $82.9 \mtiny{\pm 0.5}$ & $59.9 \mtiny{\pm 0.6}$ & $70.8 \mtiny{\pm 0.6}$ & $91.1 \mtiny{\pm 0.5}$ & $51.9 \mtiny{\pm 0.4}$ & $61.7 \mtiny{\pm 0.5}$ & $58.1 \mtiny{\pm 0.1}$ & $31.4 \mtiny{\pm 0.2}$ \\
& \textbf{LoRSU} & $75.6 \mtiny{\pm 0.6}$ & $63.7 \mtiny{\pm 0.5}$ & $82.9 \mtiny{\pm 0.4}$ & $60.5 \mtiny{\pm 0.4}$ & $73.4 \mtiny{\pm 0.8}$ & $90.7 \mtiny{\pm 0.5}$ & $51.7 \mtiny{\pm 0.4}$ & $61.6 \mtiny{\pm 0.9}$ & $58.7 \mtiny{\pm 0.2}$ & $32.2 \mtiny{\pm 0.3}$ \\
\midrule
\multirow{3}{*}{\textbf{CL-50}} & \textbf{LoRSU-Rand} & $75.4 \mtiny{\pm 0.1}$ & $66.8 \mtiny{\pm 0.2}$ & $82.2 \mtiny{\pm 0.2}$ & $59.2 \mtiny{\pm 0.3}$ & $71.7 \mtiny{\pm 0.0}$ & $90.6 \mtiny{\pm 0.2}$ & $51.9 \mtiny{\pm 0.1}$ & $61.7 \mtiny{\pm 0.1}$ & $58.3 \mtiny{\pm 0.1}$ & $31.8 \mtiny{\pm 0.1}$ \\
& \textbf{LoRSU-F} & $74.8 \mtiny{\pm 0.2}$ & $66.5 \mtiny{\pm 0.4}$ & $82.3 \mtiny{\pm 0.4}$ & $59.6 \mtiny{\pm 0.0}$ & $73.5 \mtiny{\pm 0.3}$ & $90.9 \mtiny{\pm 0.1}$ & $51.9 \mtiny{\pm 0.0}$ & $62.1 \mtiny{\pm 0.1}$ & $58.9 \mtiny{\pm 0.0}$ & $31.5 \mtiny{\pm 0.1}$ \\
& \textbf{LoRSU} & $75.7 \mtiny{\pm 0.0}$ & $72.5 \mtiny{\pm 0.0}$ & $82.0 \mtiny{\pm 0.2}$ & $59.4 \mtiny{\pm 0.1}$ & $72.4 \mtiny{\pm 0.2}$ & $90.5 \mtiny{\pm 0.3}$ & $51.7 \mtiny{\pm 0.3}$ & $61.4 \mtiny{\pm 0.2}$ & $58.3 \mtiny{\pm 0.1}$ & $31.7 \mtiny{\pm 0.0}$ \\
\bottomrule
\end{tabular}
\endgroup
\end{small}
\end{center}
\end{table}


\begin{table}
\caption{Comparison of the importance of choosing a small subset of attention heads. \emph{LoRSU-RAND-V-CLIP} randomly chooses 2 heads to fine-tune, \emph{LoRSU-F} fine-tunes all the available heads, and our baseline \emph{LoRSU} that chooses the top-2 attentions heads. We report the accuracy scores (\%) for LLaVA with the pretrained or fine-tuned CLIP CLIP-L-14. All baselines use \textbf{AIR} dataset for fine-tuning the vision encoder(the LLM remains frozen). We include error bars over 3 runs.}
 \label{table:lorsu_attn_aircraft_clip}
\begin{center}
\begin{small}
\begingroup
\setlength{\tabcolsep}{2.0pt}
\begin{tabular}{l c c c c c c c c c c c}
\toprule
 & & \multicolumn{9}{c}{\textbf{VQA Datasets (Acc \%)}}  \\
\cmidrule(lr){3-12}
\textbf{Setting} & \textbf{FT Method}  & \textbf{GTS} & \textbf{TSI} & \textbf{CAn} & \textbf{AIR} & \textbf{ESAT} & \textbf{DALLE} & \textbf{VSR} & \textbf{HM} & \textbf{MMVP} & \textbf{VisOnly} \\
\midrule
 & \textbf{Zr-Shot} & $75.6$ & $53.1$ & $82.7$ & $60.4$ & $76.1$ & $91.1$ & $51.5$ & $61.2$ & $58.0$ & $31.3$ \\
\midrule
\multirow{3}{*}{\textbf{CL-5}} & \textbf{LoRSU-Rand} & $75.0 \mtiny{\pm 1.5}$ & $53.4 \mtiny{\pm 0.6}$ & $82.3 \mtiny{\pm 0.9}$ & $63.6 \mtiny{\pm 0.7}$ & $73.5 \mtiny{\pm 0.9}$ & $91.9 \mtiny{\pm 1.0}$ & $51.5 \mtiny{\pm 0.9}$ & $62.1 \mtiny{\pm 1.2}$ & $58.8 \mtiny{\pm 0.3}$ & $31.9 \mtiny{\pm 0.3}$ \\
& \textbf{LoRSU-F} & $75.7 \mtiny{\pm 1.2}$ & $53.1 \mtiny{\pm 0.9}$ & $82.8 \mtiny{\pm 1.0}$ & $65.0 \mtiny{\pm 1.5}$ & $75.0 \mtiny{\pm 0.6}$ & $91.6 \mtiny{\pm 1.1}$ & $51.7 \mtiny{\pm 1.5}$ & $61.8 \mtiny{\pm 0.7}$ & $57.5 \mtiny{\pm 0.4}$ & $31.6 \mtiny{\pm 0.4}$ \\
& \textbf{LoRSU} & $76.1 \mtiny{\pm 0.8}$ & $53.4 \mtiny{\pm 0.8}$ & $82.8 \mtiny{\pm 0.9}$ & $65.1 \mtiny{\pm 0.9}$ & $75.9 \mtiny{\pm 1.4}$ & $91.6 \mtiny{\pm 0.6}$ & $51.6 \mtiny{\pm 0.9}$ & $62.1 \mtiny{\pm 1.5}$ & $58.9 \mtiny{\pm 0.4}$ & $31.6 \mtiny{\pm 0.4}$ \\
\midrule
\multirow{3}{*}{\textbf{CL-20}} & \textbf{LoRSU-Rand} & $74.1 \mtiny{\pm 0.6}$ & $53.0 \mtiny{\pm 0.3}$ & $81.3 \mtiny{\pm 0.8}$ & $64.3 \mtiny{\pm 0.7}$ & $73.0 \mtiny{\pm 0.5}$ & $91.1 \mtiny{\pm 0.8}$ & $51.6 \mtiny{\pm 0.9}$ & $62.1 \mtiny{\pm 0.7}$ & $57.0 \mtiny{\pm 0.2}$ & $31.3 \mtiny{\pm 0.2}$ \\
& \textbf{LoRSU-F} & $75.3 \mtiny{\pm 0.3}$ & $53.9 \mtiny{\pm 0.7}$ & $81.5 \mtiny{\pm 0.6}$ & $64.9 \mtiny{\pm 1.0}$ & $74.6 \mtiny{\pm 0.6}$ & $91.6 \mtiny{\pm 0.8}$ & $51.8 \mtiny{\pm 0.6}$ & $62.1 \mtiny{\pm 0.9}$ & $59.6 \mtiny{\pm 0.1}$ & $31.6 \mtiny{\pm 0.2}$ \\
& \textbf{LoRSU} & $76.1 \mtiny{\pm 0.7}$ & $53.0 \mtiny{\pm 0.7}$ & $81.3 \mtiny{\pm 0.7}$ & $66.2 \mtiny{\pm 0.6}$ & $74.8 \mtiny{\pm 0.8}$ & $91.3 \mtiny{\pm 0.9}$ & $51.8 \mtiny{\pm 0.6}$ & $62.1 \mtiny{\pm 0.9}$ & $56.8 \mtiny{\pm 0.3}$ & $31.8 \mtiny{\pm 0.2}$ \\
\midrule
\multirow{3}{*}{\textbf{CL-50}} & \textbf{LoRSU-Rand} & $74.5 \mtiny{\pm 0.2}$ & $52.7 \mtiny{\pm 0.2}$ & $80.2 \mtiny{\pm 0.0}$ & $67.6 \mtiny{\pm 0.1}$ & $71.3 \mtiny{\pm 0.4}$ & $91.0 \mtiny{\pm 0.2}$ & $51.5 \mtiny{\pm 0.3}$ & $62.2 \mtiny{\pm 0.4}$ & $57.4 \mtiny{\pm 0.1}$ & $31.4 \mtiny{\pm 0.1}$ \\
& \textbf{LoRSU-F} & $75.1 \mtiny{\pm 0.1}$ & $52.6 \mtiny{\pm 0.1}$ & $81.3 \mtiny{\pm 0.2}$ & $69.7 \mtiny{\pm 0.3}$ & $71.6 \mtiny{\pm 0.3}$ & $91.4 \mtiny{\pm 0.3}$ & $51.7 \mtiny{\pm 0.2}$ & $61.7 \mtiny{\pm 0.2}$ & $58.2 \mtiny{\pm 0.1}$ & $31.6 \mtiny{\pm 0.0}$ \\
& \textbf{LoRSU} & $75.4 \mtiny{\pm 0.1}$ & $52.5 \mtiny{\pm 0.2}$ & $81.6 \mtiny{\pm 0.3}$ & $68.5 \mtiny{\pm 0.1}$ & $72.8 \mtiny{\pm 0.4}$ & $91.1 \mtiny{\pm 0.3}$ & $51.9 \mtiny{\pm 0.4}$ & $62.2 \mtiny{\pm 0.2}$ & $59.2 \mtiny{\pm 0.1}$ & $31.0 \mtiny{\pm 0.1}$ \\
\bottomrule
\end{tabular}
\endgroup
\end{small}
\end{center}
\end{table}


\begin{table}
\caption{Comparison of the importance of choosing a small subset of attention heads. \emph{LoRSU-RAND-V-CLIP} randomly chooses 2 heads to fine-tune, \emph{LoRSU-F} fine-tunes all the available heads, and our baseline \emph{LoRSU} that chooses the top-2 attentions heads. We report the accuracy scores (\%) for LLaVA with the pretrained or fine-tuned CLIP CLIP-L-14. All baselines use \textbf{ESAT} dataset for fine-tuning the vision encoder(the LLM remains frozen). We include error bars over 3 runs.}
 \label{table:lorsu_attn_eurosat_clip}
\begin{center}
\begin{small}
\begingroup
\setlength{\tabcolsep}{2.0pt}
\begin{tabular}{l c c c c c c c c c c c}
\toprule
 & & \multicolumn{9}{c}{\textbf{VQA Datasets (Acc \%)}}  \\
\cmidrule(lr){3-12}
\textbf{Setting} & \textbf{FT Method}  & \textbf{GTS} & \textbf{TSI} & \textbf{CAn} & \textbf{AIR} & \textbf{ESAT} & \textbf{DALLE} & \textbf{VSR} & \textbf{HM} & \textbf{MMVP} & \textbf{VisOnly} \\
\midrule
 & \textbf{Zr-Shot} & $75.6$ & $53.1$ & $82.7$ & $60.4$ & $76.1$ & $91.1$ & $51.5$ & $61.2$ & $58.0$ & $31.3$ \\
\midrule
\multirow{3}{*}{\textbf{CL-5}} & \textbf{LoRSU-Rand} & $76.4 \mtiny{\pm 0.9}$ & $53.3 \mtiny{\pm 0.7}$ & $82.6 \mtiny{\pm 0.9}$ & $60.9 \mtiny{\pm 1.0}$ & $81.4 \mtiny{\pm 1.4}$ & $91.6 \mtiny{\pm 1.2}$ & $51.6 \mtiny{\pm 0.9}$ & $61.3 \mtiny{\pm 0.8}$ & $58.4 \mtiny{\pm 0.3}$ & $31.4 \mtiny{\pm 0.3}$ \\
& \textbf{LoRSU-F} & $76.3 \mtiny{\pm 0.8}$ & $53.5 \mtiny{\pm 0.8}$ & $82.4 \mtiny{\pm 1.4}$ & $60.9 \mtiny{\pm 0.7}$ & $82.8 \mtiny{\pm 1.4}$ & $91.9 \mtiny{\pm 1.2}$ & $51.5 \mtiny{\pm 1.2}$ & $61.2 \mtiny{\pm 0.8}$ & $57.6 \mtiny{\pm 0.4}$ & $31.4 \mtiny{\pm 0.3}$ \\
& \textbf{LoRSU} & $76.2 \mtiny{\pm 1.0}$ & $53.6 \mtiny{\pm 0.6}$ & $82.4 \mtiny{\pm 1.0}$ & $60.9 \mtiny{\pm 0.6}$ & $82.8 \mtiny{\pm 1.2}$ & $91.5 \mtiny{\pm 0.5}$ & $51.7 \mtiny{\pm 0.9}$ & $61.6 \mtiny{\pm 0.7}$ & $57.6 \mtiny{\pm 0.3}$ & $31.7 \mtiny{\pm 0.4}$ \\
\midrule
\multirow{3}{*}{\textbf{CL-20}} & \textbf{LoRSU-Rand} & $75.6 \mtiny{\pm 0.6}$ & $52.9 \mtiny{\pm 0.6}$ & $82.7 \mtiny{\pm 0.7}$ & $60.6 \mtiny{\pm 0.6}$ & $82.3 \mtiny{\pm 0.6}$ & $91.6 \mtiny{\pm 0.7}$ & $51.7 \mtiny{\pm 0.7}$ & $61.7 \mtiny{\pm 0.8}$ & $58.3 \mtiny{\pm 0.3}$ & $31.7 \mtiny{\pm 0.1}$ \\
& \textbf{LoRSU-F} & $75.6 \mtiny{\pm 0.7}$ & $53.3 \mtiny{\pm 0.3}$ & $82.8 \mtiny{\pm 0.9}$ & $60.4 \mtiny{\pm 0.7}$ & $83.1 \mtiny{\pm 0.6}$ & $92.0 \mtiny{\pm 0.8}$ & $51.7 \mtiny{\pm 0.3}$ & $61.3 \mtiny{\pm 0.6}$ & $59.1 \mtiny{\pm 0.3}$ & $31.4 \mtiny{\pm 0.3}$ \\
& \textbf{LoRSU} & $75.2 \mtiny{\pm 0.5}$ & $53.4 \mtiny{\pm 0.4}$ & $83.0 \mtiny{\pm 0.5}$ & $60.7 \mtiny{\pm 0.8}$ & $82.7 \mtiny{\pm 0.7}$ & $91.6 \mtiny{\pm 0.3}$ & $51.9 \mtiny{\pm 0.9}$ & $61.6 \mtiny{\pm 0.4}$ & $58.4 \mtiny{\pm 0.1}$ & $31.3 \mtiny{\pm 0.3}$ \\
\midrule
\multirow{3}{*}{\textbf{CL-50}} & \textbf{LoRSU-Rand} & $75.7 \mtiny{\pm 0.3}$ & $53.7 \mtiny{\pm 0.3}$ & $82.9 \mtiny{\pm 0.1}$ & $60.0 \mtiny{\pm 0.1}$ & $81.4 \mtiny{\pm 0.4}$ & $92.0 \mtiny{\pm 0.2}$ & $51.7 \mtiny{\pm 0.3}$ & $61.7 \mtiny{\pm 0.3}$ & $58.8 \mtiny{\pm 0.1}$ & $31.6 \mtiny{\pm 0.1}$ \\
& \textbf{LoRSU-F} & $75.7 \mtiny{\pm 0.2}$ & $53.5 \mtiny{\pm 0.1}$ & $82.4 \mtiny{\pm 0.3}$ & $60.3 \mtiny{\pm 0.0}$ & $80.9 \mtiny{\pm 0.2}$ & $92.1 \mtiny{\pm 0.2}$ & $51.7 \mtiny{\pm 0.1}$ & $61.5 \mtiny{\pm 0.3}$ & $57.4 \mtiny{\pm 0.1}$ & $31.2 \mtiny{\pm 0.0}$ \\
& \textbf{LoRSU} & $75.4 \mtiny{\pm 0.2}$ & $53.8 \mtiny{\pm 0.2}$ & $83.0 \mtiny{\pm 0.3}$ & $60.0 \mtiny{\pm 0.4}$ & $82.9 \mtiny{\pm 0.4}$ & $92.1 \mtiny{\pm 0.4}$ & $51.9 \mtiny{\pm 0.0}$ & $61.4 \mtiny{\pm 0.0}$ & $57.5 \mtiny{\pm 0.1}$ & $31.3 \mtiny{\pm 0.1}$ \\
\bottomrule
\end{tabular}
\endgroup
\end{small}
\end{center}
\end{table}
